Physical Adversarial Attacks For Camera-based Smart Systems: Current Trends, Categorization, Applications, Research Challenges, and Future Outlook

In this paper, we present a comprehensive survey of the current trends focusing specifically on physical adversarial attacks. We aim to provide a thorough understanding of the concept of physical adversarial attacks, analyzing their key characteristics and distinguishing features. Furthermore, we explore the specific requirements and challenges associated with executing attacks in the physical world. Our article delves into various physical adversarial attack methods, categorized according to their target tasks in different applications, including classification, detection, face recognition, semantic segmentation and depth estimation. We assess the performance of these attack methods in terms of their effectiveness, stealthiness, and robustness. We examine how each technique strives to ensure the successful manipulation of DNNs while mitigating the risk of detection and withstanding real-world distortions. Lastly, we discuss the current challenges and outline potential future research directions in the field of physical adversarial attacks. We highlight the need for enhanced defense mechanisms, the exploration of novel attack strategies, the evaluation of attacks in different application domains, and the establishment of standardized benchmarks and evaluation criteria for physical adversarial attacks. Through this comprehensive survey, we aim to provide a valuable resource for researchers, practitioners, and policymakers to gain a holistic understanding of physical adversarial attacks in computer vision and facilitate the development of robust and secure DNN-based systems.

==> other_tasks.tex <==
\section{Physical Attacks On Other Tasks}

\subsection{Attacks on Crowd Counting}
Crowd counting is a crucial task in computer vision that aims to estimate the number of people in images or videos. It has significant applications in areas such as public safety, traffic control, and crowd management. Jiang et al. \cite{jiang2020attention} introduced the concept of \textbf{Perceptual Adversarial Patch (PAP)} as a method to attack crowd counting systems in real-world scenarios. The objective of PAP is to generate adversarial patch perturbations that maximize the model loss, leading to an overestimation of the crowd count by the targeted victim model.

The effectiveness of PAP has been demonstrated through experiments, showing that it can cause the victim model to overestimate the crowd count by up to 100 individuals in 80\% of the samples. However, it should be noted that PAP does not prioritize stealthiness in its design, focusing primarily on maximizing the attack effectiveness.

To enhance the robustness of the attack, PAP incorporates attention mechanisms, enabling it to capture scale and position perceptions. This enhances its performance across multiple crowd counting models with varying structures. Furthermore, PAP demonstrates adaptability across different datasets and maintains its effectiveness even in the presence of complex backgrounds. These characteristics make PAP a powerful tool for attacking crowd counting systems, potentially posing threats to public safety measures.

\subsection{Attacks on Autonomous driving}


\subsection{Lane Detection}
